Sample-Efficient Linear Representation Learning from Non-IID Non-Isotropic Data

A powerful concept behind much of the recent progress in machine learning is the extraction of common features across data from heterogeneous sources or tasks. Intuitively, using all of one's data to learn a common representation function benefits both computational effort and statistical generalization by leaving a smaller number of parameters to fine-tune on a given task. Toward theoretically grounding these merits, we propose a general setting of recovering linear operators $M$ from noisy vector measurements $y = Mx + w$, where the covariates $x$ may be both non-i.i.d. and non-isotropic. We demonstrate that existing isotropy-agnostic representation learning approaches incur biases on the representation update, which causes the scaling of the noise terms to lose favorable dependence on the number of source tasks. This in turn can cause the sample complexity of representation learning to be bottlenecked by the single-task data size. We introduce an adaptation, $\texttt{De-bias & Feature-Whiten}$ ($\texttt{DFW}$), of the popular alternating minimization-descent scheme proposed independently in Collins et al., (2021) and Nayer and Vaswani (2022), and establish linear convergence to the optimal representation with noise level scaling down with the $\textit{total}$ source data size. This leads to generalization bounds on the same order as an oracle empirical risk minimizer. We verify the vital importance of $\texttt{DFW}$ on various numerical simulations. In particular, we show that vanilla alternating-minimization descent fails catastrophically even for iid, but mildly non-isotropic data. Our analysis unifies and generalizes prior work, and provides a flexible framework for a wider range of applications, such as in controls and dynamical systems.

==> tex/IL_numerical_results.tex <==
\subsection{Imitation learning}

We now focus on the problem of learning a linear quadratic regulator (LQR) controller, denoted as $K^{(H+1)} = F^{(H+1)}\star \Phi\star$. To achieve this, we begin by computing a shared low-rank representation for all tasks $h \in [H+1]$ by leveraging data from expert controllers $K^{(1)}, K^{(2)},\ldots, K^{(H)}$. In this context, we consider the following discrete-time linear time-invariant dynamical system:
\begin{align*}
    x^{(h)}[t+1]=Ax^{(h)}[t] + Bu^{(h)}[t], \;\ t=0,1,\ldots,T-1,
\end{align*}
with $n_x$ states and $n_u$ inputs, for all $h \in [H+1]$, where $u^{(h)}[t] = K^{(h)}x^{(h)}[t] + z^{(h)}[t]$, with $z^{(h)}[t] \sim \mathcal{N}(0,I_{d_u})$ being the input noise. In our setting, instead of directly observing the state, we obtain a high-dimensional observation that is derived from an injective linear function of the state. Specifically, we assume that $y^{(h)}[t] = Gx^{(h)}[t] + w^{(h)}[t] $, where $G \in \mathbb{R}^{25\times 4}$ represents the high-dimensional linear mapping. The matrix $G$ is generated by performing a \texttt{thin\_svd} operation on a random matrix with values drawn from a normal distribution $\mathcal{N}(0,1)$. For the first $H$ expert controllers, we collect a dataset $\{\{y^{(h)}[h],u^{(h)}[t]\}_{t=0}^{T-1}\}_{h=1}^H$, where the observation follows the dynamics:
\begin{align*}
    y^{(h)}[t] = (\tilde{A} + \tilde{B}\Tilde{K}^{(h)})y[t] + \Tilde{B}z^{(h)}[t] + w^{(h)}[t]
\end{align*}
with $\Tilde{A} = GAG^{\dagger}$, $\Tilde{B}=GB$, $\tilde{K}^{(h)} = K^{(h)}G^{\dagger}$, and process noise $w^{(h)}[t] \sim \mathcal{N}(0,\Sigma_w)$. To generate the collection of stabilizing LQR controllers $K^{(1)}, K^{(2)}, \ldots, K^{(H+1)}$, we first set different cost matrices, $R = \frac{1}{4}I_{n_u}$ and $Q^{(h)}=\alpha^{(h)}I_{n_x}$, where $\alpha^{(h)} \in \texttt{logspace}(0,3, H+1)$, and use it to solve the Discrete Algebraic Ricatti equation (DARE): $P^{(h)} = A^\top P^{(h)}A^\top + A^\top P^{(h)} B(B^\top P^{(h)}B + R)^{-1}B^\top P^{(h)} A + Q^{(h)}$, and compute $K^{(h)}=-(B^\top P^{(h)}B + R)^{-1}B^\top P^{(h)} A$, for all $h \in [H+1]$. For the simulations, we set the number of states as $n_x=4$ and the number of inputs as $n_u=2$. The system matrices $A$ and $B$ are generated randomly, with elements drawn from a uniform distribution. The trajectory length $T=75$ is the same across all tasks. The shared representation is initialized from a random rotation of the true representation, denoted as $\Phi_\star = G^{\dagger}$.



\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{tex/Figures/sysID/linear_sysid_random_matrix.pdf}
         \caption{}
         \label{fig:sysID}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{tex/Figures/IL/imitation_learning.pdf}
         \caption{}
         \label{fig:IL}
     \end{subfigure}
        \caption{Subspace distance between the updated and ground truth representation with respect to the number of iterations. Comparison between the single-task and multiple-tasks settings with Algorithm \ref{alg: multi-task alt min descent} and the multi-task operator recovery with Alt. Minimization-Descent algorithm (FedRep in \cite{collins2021exploiting}). (a) System identification. (b) Imitation learning}
        \label{fig:linear_regression_varying_beta}
\end{figure}

==> tex/matrix_sensing_alg.tex <==
\section{Alternating Optimization for Multi-Task Linear Inverse Problems}

Let us the consider a simple multi-task linear inverse problem, where the aim is to recover generating linear operators from $(z,y)$ pairs, $z \in \R^{d_z}$, $y \in \R^{d_y}$ satisfying
\begin{align*}
    y^{(h)} = M^{(h)} z^{(h)} + w,\quad w \iidsim \calN(0, \sigma^2 I),
\end{align*}
where $M^{(h)} = F^{(h)} \Phi$ for all $h \in [H]$, $\Phi \in \R^{r \times d_z}$, are the task-specific linear operators to be learned. Let us assume for convenience that $(x^{(h)}, y^{(h)}) \iidsim \calD(h)$ (\blue{$(z^{(h)}, y^{(h)}) \iidsim \calD(h)$}).  \red{The broad (vague) question here comes in two parts:
\begin{enumerate}
    \item what type of alternating optimization scheme provably converges to the optimal solution, and complementarily...
    
    \item what assumptions must be made on the conditioning of the matrices to guarantee recovery? (Extensions of matrix restricted isometry / null space property / incoherence etc)
    
\end{enumerate}
}
Let us start with a simple alternating descent psuedo-algorithm, a very close variant of which we used to \textit{successfully} generate the numerical results in \citep{zhang2022multi} (which suggests it's sound empirically).
\begin{algorithm}[H]
    \caption{Alt Descent for Linear Inverse Problems}
    \label{alg: multi-task LIP}
    \begin{algorithmic}[1]
        \State \textbf{Input:} rank overestimate $r$, step size $\eta$.
        \State \textbf{Initialize} $F_0^{(h)} \iidsim \calN(0,1)^{d_y \times r}$, $\Phi_0 \sim \calN(0,1)^{r \times d_z}$.
        \For {$k = 1, \dots, K$}
            \For {$h \in [H]$}
                \State Sample $\curly{z^{(h)}_{k,i}, y^{(h)}_{k,i}}_{i=1}^N \iidsim \calD(h)^{N}$.
                % \State $F^{(h)}_k \leftarrow F^{(h)}_{k-1} + \eta \pder{}{F} \frac{1}{N}\sum_{i=1}^N \norm{y^{(h)}_{k,i} - F \Phi_{k-1} z^{(h)}_{k,i}}^2$. \Comment{update task weights}
                \State $F^{(h)}_k \leftarrow \argmin_{F} \frac{1}{2N}\sum_{i=1}^N \norm{y^{(h)}_{k,i} - F \Phi_{k-1} z^{(h)}_{k,i}}^2$. \Comment{update task weights}
                \State $\Phi_k|_h \leftarrow \Phi_{k-1} - \eta \pder{}{\Phi} \frac{1}{2N}\sum_{i=1}^N \norm{y^{(h)}_{k,i} - F^{(h)}_{k} \Phi_{k-1} z^{(h)}_{k,i}}^2$. \Comment{task-conditioned rep update}
            \EndFor
            \State $\_\_, \Phi_k \leftarrow \texttt{thin\_RQ}\paren{\frac{1}{H} \sum_{h=1}^{H} \Phi_k|_h}$. \Comment{aggregate rep updates and normalize via (thin) RQ decomp}
        \EndFor
    \end{algorithmic}
\end{algorithm}
Minus a method-of-moments initialization of the representation, \Cref{alg: multi-task LIP} is essentially the linear inverse problem analog to \texttt{FedRep}, which is specified to linear regression (which can be embedded as a LIP by setting $p = 1$). We note that, like in \texttt{FedRep}, the algorithm is a combination of alternating minimization and descent, where we minimize the task-specific weights in the inner loop, and perform descent on the representation. This is a sensible formulation for the online control set-up.

\red{Something that is not immediately clear to me is whether a linear inverse problem is compatible with the matrix sensing framework (using embeddings that do not blow up dimension).}


\subsection{Towards a convergence proof for \Cref{alg: multi-task LIP}}

\red{SOME IMPORTANT NOTES:}
\begin{itemize}
    \item After reading \texttt{FedRep}, I noticed that their setting/analysis \textit{does not} include label noise ($w$ in the notation here). In other words, the only randomness comes from the distribution of the covariates ($z$ here). This is actually rather suspect when it comes the claims in their paper, since the multi-task linear regression problem formulation they borrow from \cite{tripuraneni2021provable, du2020few} crucially involves the label noise, otherwise linear regression is trivial as a statistical problem: under non-degeneracy conditions of $z$, $d_z$ samples is sufficient to precisely invert any tall matrix $M$ (similarly for wide matrices). After carefully reading the analysis in \texttt{FedRep}, this invertability property is key in their analysis showing that the common representation $\Phi_k$ converges to the optimal $\Phi^*$ linearly $k = \calO(\log(1/\varepsilon))$. This linear convergence should have set off some alarms, since this is much faster than any usual statistical rates for least squares-type problems, usually topping out at $k \approx \calO(1/\varepsilon)$.
    
    This is fine if it weren't for the fact that the faster convergence is stated as a contribution over the alternating minimization approach in \cite{tripuraneni2021provable}, which has a convergence rate of $\tilde\calO(1/\varepsilon^2)$--however, this rate is under the presence of label noise. Therefore, that rate is reasonable, since (disregarding dimensionality dependence) this corresponds to the CLT convergence / usual ``slow'' rate of $\calO(1/\sqrt{N})$.
    
    \red{Update:} 
    
    \item I've come to realize that finagling the problem to pose it as a matrix sensing problem might be a wasted effort -- so far a direct approach that I've been taking seems to be working.
    
\end{itemize}

Now for the proof attempt. Recall the linear inverse problem formulation from earlier in the section, where we have
\[
y^{(h)} = F^{(h)} \Phi z^{(h)} + w,\quad w \iidsim \calN(0, \sigma^2 I),
\]
for tasks indexed by $h = 1, \dots, H$. We consider a arbitrary iteration in \Cref{alg: multi-task LIP}. In particular, we have task-specific weight matrices $F^{(h)}$, and a common representation $\hat \Phi$ (with orthonormal rows). The weights are updated via a new batch of task-specific data $\curly{(z^{(h)}_i, y^{(h)}_i)}_{i=1}^N$
\begin{equation}
    F^{(h)}_+ = \argmin_F \frac{1}{2N} \sum_{i=1}^N \norm{y^{(h)}_i - F \hat\Phi z^{(h)}_i }^2,\quad h \in [H].
\end{equation}
The representation is then updated by a gradient descent step and applying an RQ decomposition, fixing $\Fh_+$
\begin{equation}
    R\hat\Phi_+ = \hat\Phi - \frac{\eta}{2HN} \sum_{h=1}^H \sum_{i=1}^N \pder{}{\Phi} \norm{y^{(h)}_i - \Fh_+ \hat\Phi z^{(h)}_i }^2.
\end{equation}
The weight update is a standard least squares problem. Using matrix derivative identities from \cite{petersen2008matrix}, we solve for $F^{(h)}_+$ via
\begin{align*}
    \b0 &= \pder{}{F} \frac{1}{N} \sum_{i=1}^N \norm{y^{(h)}_i - F \hat\Phi z^{(h)}_i }^2 = -\frac{1}{N}\sum_{i=1}^N \yhi {\zhi}^\top \hat\Phi^\top +   \frac{1}{N}\sum_{i=1}^N F \hat\Phi \zhi {\zhi}^\top \hat\Phi^\top \\
    \implies \Fh_+ &= \sum_{i=1}^N \yhi \paren{\hat\Phi \zhi}^\top \paren{\sum_{i=1}^N \hat\Phi \zhi \paren{\hat\Phi\zhi}^\top }^{-1} \\
    &= \sum_{i=1}^N \Fh_\star \Phi_\star \zhi \paren{\hat\Phi \zhi}^\top \paren{\sum_{i=1}^N \hat\Phi \zhi \paren{\hat\Phi\zhi}^\top }^{-1} + \sum_{i=1}^N \whi \paren{\hat\Phi \zhi}^\top \paren{\sum_{i=1}^N \hat\Phi \zhi \paren{\hat\Phi\zhi}^\top }^{-1}.
\end{align*}
We observe that since $\whi$ is i.i.d.\ zero-mean noise, and by defining $\vhi := \hat\Phi \zhi \in \R^r$, the second term in the expression of $\Fh_+$ is a matrix-valued self-normalized martingale, for which we can derive concentration bounds using, e.g.\, tools from \citet[Appendix B]{zhang2022multi}. A good sign is that since $\vhi$ takes values in $\R^r$, the concentration bounds will inherit the low-dimensionality. We note that since the analysis in \cite{collins2021exploiting} does not have additive noise, their analogous expression for $\Fh_+$ only involves the first term. Now simply adding and subtracting a term, we can further write
\begin{align*}
    \Fh_+ &= \sum_{i=1}^N \Fh_\star \Phi_\star \zhi \vhi^\top \paren{\sum_{i=1}^N \vhi \vhi^\top }^{-1} \pm \sum_{i=1}^N \Fh_\star \Phi_\star \hat\Phi^\top \vhi\vhi^\top \paren{\sum_{i=1}^N \vhi \vhi^\top }^{-1} \\
    &\quad + \sum_{i=1}^N \whi \vhi^\top \paren{\sum_{i=1}^N \vhi \vhi^\top }^{-1} \\
    &= \underbrace{\Fh_\star \Phi_\star \hat\Phi^\top}_{\approx \Fh_\star} + \underbrace{\Fh_\star \Phi_\star \paren{I_{d_z} - \hat \Phi^\top \hat \Phi} \paren{\sum_{i=1}^N \zhi \zhi^\top } \hat\Phi^\top \paren{\sum_{i=1}^N \vhi \vhi^\top }^{-1}}_{\text{``Error term'': scales with }\mathrm{dist}(\hat \Phi, \Phi_\star), \text{ goes to }0\text{ when }\hat\Phi \to \Phi_\star} + \underbrace{\sum_{i=1}^N \whi \vhi^\top \paren{\sum_{i=1}^N \vhi \vhi^\top }^{-1}}_{\text{Self-norm.\ ``noise term'': }\to_N 0}.
\end{align*}
We have therefore decomposed the weight update into three terms, which clearly delineate a term that approaches the true weight $\Fh_\star$, an approximation error term, and a stochastic noise term.

Now expanding out the representation gradient, we have
\begin{align*}
    \frac{1}{2HN} \sum_{h=1}^H \sum_{i=1}^N \pder{}{\Phi} \norm{y^{(h)}_i - \Fh_+ \hat\Phi z^{(h)}_i }^2 &= \frac{1}{HN} \sum_{h=1}^H \sum_{i=1}^N -{\Fh_+}^\top \yhi {\zhi}^\top + {\Fh_+}^\top \Fh_+ \hat\Phi \zhi {\zhi}^\top \\
    &= \blue{-} \frac{1}{HN} \sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \paren{\Fh_+ \hat\Phi-\Fh_\star \Phi_\star} \zhi\zhi^\top \\
    &\quad \blue{-} \frac{1}{HN}\sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \whi \zhi^\top.
\end{align*}
Recall that since $\hat\Phi$ is a matrix with orthonormal rows, $\calP_{\hat\Phi^{\perp}} := I_{d_z} - \hat \Phi^\top \hat \Phi$ is the projection matrix onto the orthogonal complement of the subspace spanned by the rows of $\hat\Phi$. Plugging this back into the representation update, we have
\begin{align*}
    R\hat\Phi_+ &= \hat\Phi - \frac{\eta}{HN} \sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \paren{\Fh_+ \hat\Phi-\Fh_\star \Phi_\star} \zhi\zhi^\top - \frac{\eta}{HN}\sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \whi \zhi^\top \\
    % &= \hat\Phi - \frac{\eta}{HN} \sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \paren{\Fh_+ \hat\Phi-\Fh_\star \Phi_\star} {\Phi_\star^\perp}^{\top}- \frac{\eta}{HN}\sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \whi \zhi^\top \\
    % &= \paren{I - \frac{\eta}{HN} \sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \Fh_+ }\hat\Phi {\Phi_\star^\perp}^{\top} - \frac{\eta}{HN}\sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \whi \zhi^\top\\
    % &= \hat \Phi - \frac{\eta}{HN}\sum_{h=1}^H {\Fh_+}^\top \Bigg( \Fh_\star\Phi_\star \hat\Phi^\top \hat\Phi - \Fh_\star\Phi_\star + \Fh_\star \Phi_\star \calP_{\hat\Phi^{\perp}} \paren{\sum_i \zhi \zhi^\top} \hat\Phi^\top \paren{\sum_i \vhi\vhi^\top}^{-1}\hat\Phi   \\
    % &\qquad\qquad\qquad\qquad\qquad +  \sum_i \whi \vhi^\top \paren{\sum_i \vhi\vhi^\top}^{-1} \hat\Phi \Bigg) \paren{\sum_i \zhi\zhi^\top} \\
    % &\quad \quad - \frac{\eta}{HN}\sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \whi \zhi^\top \\
    % &= \hat\Phi - \frac{\eta}{HN}\sum_{h=1}^H {\Fh_+}^\top \Bigg(-\Fh_\star \Phi_\star \calP_{\hat\Phi^\perp} + \Fh_\star \Phi_\star \calP_{\hat\Phi^\perp}  \paren{\sum_i \zhi \zhi^\top} \hat\Phi^\top \hat \Phi  \paren{\sum_i \zhi \zhi^\top}^{\dagger} \hat\Phi^\top \hat \Phi \\
    % &\qquad\qquad\qquad\qquad\qquad +  \sum_i \whi \vhi^\top \paren{\sum_i \vhi\vhi^\top}^{-1} \hat\Phi \Bigg) \paren{\sum_i \zhi\zhi^\top} \\
    % &\quad \quad - \frac{\eta}{HN}\sum_{h=1}^H \sum_{i=1}^N {\Fh_+}^\top \whi \zhi^\top,
\end{align*}
% where we used the following lemma to pull out $\hat\Phi$ in various places.

% \begin{lemma}

% Let $\Phi \in \R^{r \times d_x}$, be a matrix with orthonormal rows, and $Z \in \mathbb{S}^{d_x}_+$ be a positive semidefinite matrix. Assume $\Phi Z \Phi^\top$ is invertible for convenience. Then
% \begin{equation}
%     \paren{\Phi Z \Phi^\top}^{-1} = \Phi Z^{\dagger} \Phi^\top.
% \end{equation}

% \end{lemma}


% \textit{Proof:} let $Z = U\Sigma U^\top$ be the SVD of $Z$. It is easy to verify that $\Psi := \Phi U$ remains a matrix with orthonormal rows. Since $Z$ is psd, we know $Z^\dagger = U \Sigma^\dagger U^\top$, thus it suffices to verify the statement for $Z \equiv \Sigma$ a non-negative diagonal matrix. Denoting $v_i$ the rows of $\Phi$, the statement for diagonal $\Sigma$ follows by observing
% \begin{align*}
%     \Phi \Sigma^{\dagger} \Phi^\top &= \sum_{i=1}^r \sigma_i^{-1} v_i v_i^\top \\
%     \paren{\Phi \Sigma \Phi^\top}^{-1} &= \sum_{i=1}^r \sigma_i^{-1} v_i v_i^\top,
% \end{align*}
% which completes the proof. \hfill $\blacksquare$

\red{It may be notationally simpler and more informative to work out the single-task setting first.}

\section{Working out the single task/agent case}


\subsection{Why vanilla gradient descent is hard to analyze for anisotropic $z$}

\newcommand{\Phiperp}{\Phi_{\star,\perp}}

Before we worry about what task diversity conditions to pose for multi-task learning to work, let us first work out the non-trivial problem of (stochastic) bi-linear operator recovery via the proposed alternating minimization/descent algorithm, especially when the covariance of data $z_i$ is \textit{not} scaled identity, as seems to be the unifying simplification across references \citep{tripuraneni2020theory, collins2021exploiting}. Notationally, we are simply removing $h$ in our above derivations:
\[
y = F_\star \Phi_\star z + w,\quad w \iidsim \calN(0, \sigma^2 I),\quad\Phi_\star \in \calO_{k \times d_z}
\]
such that for given iterates $F,\hat\Phi$, and data batch $\curly{z_i, y_i}_{i=1}^N$ the update rules are
\begin{align*}
    F_+ &= \sum_{i=1}^N F_\star \Phi_\star z_i \paren{\hat\Phi z_i}^\top \paren{\sum_{i=1}^N \hat\Phi z_i \paren{\hat\Phi z_i}^\top }^{-1} + \sum_{i=1}^N w_i \paren{\hat\Phi z_i}^\top \paren{\sum_{i=1}^N \hat\Phi z_i \paren{\hat\Phi z_i}^\top }^{-1} \\
    R\hat\Phi_+ &= \hat\Phi - \frac{\eta}{N} \sum_{i=1}^N F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star} z_i z_i^\top - \frac{\eta}{N} \sum_{i=1}^N F_+^\top w_i z_i^\top.
\end{align*}
The canonical measure of improvement for the convergence of the representation $\hat\Phi$ is the subspace distance, i.e.
\[
\dist\paren{\Phi, \Phi_\star} := \norm{\Phi\Phiperp^\top}.
\]
Therefore, multiplying the above descent step on the right by $\Phiperp^\top$, we get
\begin{align*}
    R\hat\Phi_+\Phiperp^\top &= \hat\Phi \Phiperp^\top - \frac{\eta}{N} \sum_{i=1}^N F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}z_i z_i^\top \Phiperp^\top - \frac{\eta}{N} \sum_{i=1}^N F_+^\top w_i z_i^\top \Phiperp^\top.
\end{align*}
Notice that if $z_i \sim \calN(0,cI)$, then we can write
\begin{align*}
    R\hat\Phi_+\Phiperp^\top &= \hat\Phi \Phiperp^\top - \frac{\eta}{N}  F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}\paren{\sum_{i=1}^N z_i z_i^\top \pm c N I} \Phiperp^\top  - \frac{\eta}{N} \sum_{i=1}^N F_+^\top w_i z_i^\top \Phiperp^\top \\
    &= \hat\Phi \Phiperp^\top - c\eta F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}\Phiperp^\top - \eta F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}\paren{\frac{1}{N}\sum_{i=1}^Nz_i z_i^\top - c I} \Phiperp^\top  - \frac{\eta}{N} \sum_{i=1}^N F_+^\top w_i z_i^\top \Phiperp^\top \\
    &= \underbrace{\paren{I - c\eta F_+^\top F_+ } \hat\Phi \Phiperp^\top}_{\text{``contracting'' in sub.\ dist}} - \eta F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}\underbrace{\paren{\frac{1}{N}\sum_{i=1}^Nz_i z_i^\top - c I}}_{\text{covariance conc.\ }} \Phiperp^\top  - \frac{\eta}{N} \sum_{i=1}^N F_+^\top w_i z_i^\top \Phiperp^\top,
\end{align*}
where due to the identity covariance structure we were easily able to pull out a factor of $\hat\Phi \Phiperp^\top$ and zero out the term with $\Phi_\star \Phiperp^\top = 0$. Life is not so simple when $z_i$ are non-negotiably anisotropic, as is the case when $z_i = \bmat{x_i^\top & u_i^\top}^\top$ in sys-ID. Therefore, in general, substituting a general covariance matrix $\Sigma_z$ instead of $cI$, we instead get the nastier expression
\begin{align*}
    R\hat\Phi_+\Phiperp^\top &= \hat\Phi \Phiperp^\top - \eta  F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}\paren{\frac{1}{N}\sum_{i=1}^N z_i z_i^\top \pm   \Sigma_z} \Phiperp^\top  - \frac{\eta}{N} \sum_{i=1}^N F_+^\top w_i z_i^\top \Phiperp^\top \\
    &= \hat\Phi \Phiperp^\top - \eta  F_+^\top F_+ \hat\Phi \Sigma_z \Phiperp^\top + \eta  F_+^\top F_\star \Phi_\star \Sigma_z \Phiperp^\top \\
    &\quad - \eta F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}\paren{\frac{1}{N}\sum_{i=1}^N z_i z_i^\top  -   \Sigma_z} \Phiperp^\top  - \frac{\eta}{N} \sum_{i=1}^N F_+^\top w_i z_i^\top \Phiperp^\top,
\end{align*}
where we note that we now can't easily pull out a common factor of the subspace angle matrix $\hat\Phi \Phiperp^\top$. We zoom in on the first three terms of the descent step and consider our options--for now, we can believe the fourth and fifth terms can be controlled by concentration arguments. We now propose the following auxiliary linear algebraic lemmas.
\newcommand{\Vperp}{V_{k,\perp}}
\begin{lemma}\label{lem: diag approx}
    Let $\bV = \bmat{v_1^\top \\ \vdots \\ v_n^\top} \in \R^{n \times n}$ be an orthogonal matrix composed of (row) basis vectors $v_1, \dots, v_n$. Let us now define the subspace matrix and its orthogonal complement formed by
    \[
    V_k := \bmat{v_1^\top \\ \vdots \\ v_k^\top} \in \R^{k \times n}, \quad \Vperp := \bmat{v_{k+1}^\top \\ \vdots \\ v_n^\top} \in \R^{(n-k) \times n}.
    \]
    Then for a given psd matrix $\Sigma \succ 0$, we have
    \begin{align*}
        \norm{V_k \Sigma \Vperp^\top} &= \min_{M = V^\top \diag(\lambda) V, \;\lambda \in \R^n_+} \norm{V_k \paren{\Sigma - M} \Vperp^\top} \\
        &\leq \min_{\lambda \in \R^n_+} \norm{\bV\Sigma \bV^\top - \diag(\lambda)}.
    \end{align*}
\end{lemma}

\begin{corollary}\label{cor: identity approx bound}
    Let $\bV$, $V_k$, $\Vperp$ be defined as in \Cref{lem: diag approx}. Let $\hat V_k := \bmat{\hat v_1^\top \\ \vdots \\ \hat v_k}$ be a matrix with orthonormal rows that satisfies $\dist\paren{\hat V_k, V_k} < 1$. Then for a given psd matrix $\Sigma \succ 0$, we have the following bounds:
    \begin{align}
        \norm{V_k \Sigma \Vperp^\top} &\leq \frac{\lambda_{\max}(\Sigma) - \lambda_{\min}(\Sigma)}{2} \\
        \norm{\hat V_k \Sigma \Vperp^\top} &\leq \frac{\lambda_{\max}(\Sigma) - \lambda_{\min}(\Sigma)}{2} \paren{1 + \dist\paren{\hat V_k, V_k}}.
    \end{align}
\end{corollary}

\red{This route seems to be a dead end for now. The reason is as follows: no matter what we do, if we simply naively multiply $\Phiperp^\top$ on the right as above, then we accrue an additive factor that scales with $\frac{\lambda_{\max}(\Sigma) - \lambda_{\min}(\Sigma)}{2}$ (and is not affected by the \#data $N$). This means the limits of this analysis give us a constant bias factor for every descent step on the representation that cannot be shrunk by the size of the data batch. For now, I will put this proof direction on hold in favor of a new approach.}


\subsection{Saved by preconditioning the representation gradient}

As seen above, anisotropic data $z_i$ introduce a headache into the above analysis, where right-multiplying by the orthogonal complement $\Phiperp^\top$ gets warped by the (empirical) covariance matrix of $z_i$. Therefore, an obvious-in-hindsight way to deal with this is to change the algorithm. Instead of performing vanilla gradient descent on the representation $\hat \Phi$, we instead adjust the gradient by the inverse covariance matrix. In short, the vanilla gradient of the representation takes form
\begin{align*}
    \bG := \pder{}{\Phi} \frac{1}{N} \sum_{i=1}^N \norm{y_i - F_+ \hat \Phi z_i}^2 &=  F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star} \paren{\frac{1}{N} \sum_{i=1}^N z_i z_i^\top} + \frac{1}{N} \sum_{i=1}^N F_+^\top w_i z_i^\top,
\end{align*}
where we see on the first term ends with a pesky empirical covariance $\paren{\frac{1}{N} \sum_{i=1}^N z_i z_i^\top}$. Therefore, to counter the technical difficulties induced by this covariance factor explained in the previous section, it is natural to consider preconditioning the gradient by the inverse empirical covariance to erase that factor:
\begin{align*}
    \bH &:= \paren{F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star} \paren{\frac{1}{N} \sum_{i=1}^N z_i z_i^\top} + \frac{1}{N} \sum_{i=1}^N F_+^\top w_i z_i^\top} \paren{\frac{1}{N} \sum_{i=1}^N z_i z_i^\top}^{-1} \\
    &= F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star} + \sum_{i=1}^N F_+^\top w_i z_i^\top \paren{\sum_{i=1}^N z_i z_i^\top}^{-1},
\end{align*}
where the first term becomes a lot more palatable, and the second noise term simply goes from a matrix martingale to a self-normalized one. In terms of computation, we can solve for $\bH$ by solving the following matrix equation
\[
\bH \paren{\frac{1}{N} \sum_{i=1}^N z_i z_i^\top} = \bG,
\]
which is numerically kosher, and can in principle be parallelized easily. Therefore, for given iterates $\hat F, \hat \Phi$, we have the following updates
\begin{align*}
    F_+ &= \sum_{i=1}^N F_\star \Phi_\star z_i \paren{\hat\Phi z_i}^\top \paren{\sum_{i=1}^N \hat\Phi z_i \paren{\hat\Phi z_i}^\top }^{-1} + \sum_{i=1}^N w_i \paren{\hat\Phi z_i}^\top \paren{\sum_{i=1}^N \hat\Phi z_i \paren{\hat\Phi z_i}^\top }^{-1} \\
    R\hat\Phi_+ &= \hat \Phi - \eta \bH \\
    &= \hat\Phi - \eta F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star} - \eta \sum_{i=1}^N F_+^\top w_i z_i^\top \paren{\sum_{i=1}^N z_i z_i^\top}^{-1}.
\end{align*}
Now we may apply $\Phiperp^\top$ on both sides of the latter equation, which yields:
\begin{align*}
    R\hat\Phi_+ \Phiperp^\top &= \hat\Phi \Phiperp^\top - \eta F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}\Phiperp^\top - \eta \sum_{i=1}^N F_+^\top w_i z_i^\top \paren{\sum_{i=1}^N z_i z_i^\top}^{-1}\Phiperp^\top \\
    &= \paren{I - \eta F_+^\top F_+}\hat\Phi \Phiperp^\top - \eta \sum_{i=1}^N F_+^\top w_i z_i^\top \paren{\sum_{i=1}^N z_i z_i^\top}^{-1}\Phiperp^\top \\
    \implies \dist\paren{\hat \Phi_+, \Phi_\star} &\leq \norm{R^{-1}} \brac{\norm{I - \eta F_+^\top F_+} \dist\paren{\hat \Phi, \Phi_\star} + \eta \norm{\sum_{i=1}^N F_+^\top w_i z_i^\top \paren{\sum_{i=1}^N z_i z_i^\top}^{-1}} },
\end{align*}
which is considerably cleaner and more intuitive than the vanilla gradient descent version. There remain three broad tasks:
\begin{enumerate}
    
    \item Demonstrate $\norm{I - \eta F_+^\top F_+}$ is a contraction (with high probability).

    \item Provide a high-probability bound on the (inverse of) Gram-Schmidt factor $\norm{R^{-1}} \equiv 1/\sigma_{\min}(R)$. This should essentially follow by expanding $R R^\top = R\hat\Phi_+ \paren{R \hat\Phi_+}^\top$ via the gradient step. This bound needs to be good enough such that it doesn't outstrip the contraction rate.
    
    
    \item Bound the self-normalized martingale term $\norm{\sum_{i=1}^N F_+^\top w_i z_i^\top \paren{\sum_{i=1}^N z_i z_i^\top}^{-1}}$. This involves a covering argument, since $F_+$ is entirely dependent on $w_i, z_i$.
\end{enumerate}

\subsubsection{Bounding $\norm{I - \eta F_+^\top F_+}$}

This is rather trivial in a single-task setting. Some care will need to be taken in the multi-task setting, where we need to impose task-diversity constraints, for example to ensure
\begin{align*}
    \lambda_{\min}\paren{\frac{1}{H}\sum_{h=1}^H {\Fh_+}^\top \Fh_+} \geq \Omega\paren{1}.
\end{align*}
\red{Maybe this is precisely the task diversity assumption (on the weight matrices). On that note, I wonder whether the task diversity assumptions on the data distribution $\Sigma^{(h)}_z$ will ever come into play (as is essential in \cite{zhang2022multi}), considering we are literally preconditioning away the covariance of the data in the representation gradient.}

In any case, we recall that the least-squares weight matrix can be written as
\begin{align}
    F_+ &= F_\star \Phi_\star \hat\Phi^\top + F_\star \Phi_\star \paren{I_{d_z} - \hat \Phi^\top \hat \Phi} \paren{\sum_{i=1}^N z_i z_i^\top } \hat\Phi^\top \paren{\sum_{i=1}^N \hat\Phi z_i z_i^\top \hat\Phi^\top }^{-1} + \sum_{i=1}^N w_i z_i^\top \hat\Phi^\top\paren{\sum_{i=1}^N \hat\Phi z_i z_i^\top \hat\Phi^\top}^{-1} \nonumber\\
    &=: F_\star \Phi_\star \hat\Phi^\top + F_\star \Delta + E_N \nonumber\\
    \implies F_+^\top F_+ &= \hat\Phi \Phi_\star^\top F_\star^\top F_\star \Phi_\star \hat\Phi^\top + \Delta^\top F_\star^\top F_\star \Delta + E_N^\top E_N + \Delta^\top F_\star^\top F_\star \Phi_\star \hat\Phi^\top + \hat\Phi \Phi_\star^\top F_\star^\top F_\star \Delta + \calO\paren{E_N}, \label{eq: F'F expansion}
\end{align}
where we simply expanded $F_+^\top F_+$ and lumped all terms linear in the martingale term $E_N$ into $\calO(E_N)$. We note that for appropriately selected step size $\eta$ (which we will determine in hindsight), we are guaranteed
\[
0 \prec \eta F_+^\top F_+ \prec I,
\]
and thus
\[
\norm{I - \eta F_+^\top F_+} = 1 - 
\eta \lambda_{\min}\paren{F_+^\top F_+}.
\]
Therefore, it remains to lower bound the smallest eigenvalue of $F_+^\top F_+$ based on the expansion above. Roughly speaking, by the superadditivity of the smallest eigenvalue of symmetric matrices, since the first three terms in \eqref{eq: F'F expansion} are psd, they only serve to improve the contraction rate; the second term $\Delta^\top F_\star^\top F_\star \Delta$ will be quadratic in $\norm{\Phi_\star \paren{I - \hat\Phi^\top \Phi}} = \norm{\Phi_\star \hat\Phi_\perp^\top}_2 = \dist(\hat\Phi, \Phi_\star)$, and the third term $E_N^\top E_N$ will be of magnitude $1/N$, and therefore their benefit will be negligible in comparison to the non-psd cross terms. It therefore suffices to bound the dominant psd term $\hat\Phi \Phi_\star^\top F_\star^\top F_\star \Phi_\star \hat\Phi^\top$ and symmetric cross term $\Delta^\top F_\star^\top F_\star \Phi_\star \hat\Phi^\top + \hat\Phi \Phi_\star^\top F_\star^\top F_\star \Delta$. This is similar to the analysis in \citet[Appendix B.3]{collins2021exploiting}.
\begin{align*}
    \lambda_{\min}\paren{\hat\Phi \Phi_\star^\top F_\star^\top F_\star \Phi_\star \hat\Phi^\top} &= \min_{\norm{x} = 1} x^\top \hat\Phi \Phi_\star^\top F_\star^\top F_\star \Phi_\star \hat\Phi^\top x \\
    &\geq \lambda_{\min}\paren{F_\star^\top F_\star} \min_{\norm{x} = 1} x^\top \hat\Phi \Phi_\star^\top \Phi_\star \hat\Phi^\top x \\
    &= \lambda_{\min}\paren{F_\star^\top F_\star} \sigma_{\min}^2\paren{\Phi_\star \hat\Phi^\top}.
\end{align*}
To further lower bound $\sigma_{\min}^2\paren{\Phi_\star \hat\Phi^\top}$, we observe that
\begin{align*}
    \hat\Phi \hat\Phi^\top &= \hat\Phi \paren{\Phi_\star^\top \Phi_\star + \Phiperp^\top \Phiperp} \hat\Phi^\top \\
    \implies 1 = \lambda_{\max}(\hat\Phi \hat\Phi^\top) &\leq \lambda_{\min}\paren{\hat\Phi \Phi_\star^\top \Phi_\star \hat\Phi^\top} + \lambda_{\max}\paren{\hat\Phi \Phiperp^\top \Phiperp \hat\Phi^\top} \quad \text{Weyl's inequality} \\
    \implies \sigma_{\min}^2\paren{\Phi_\star \hat\Phi^\top} &\geq 1 - \sigma_{\min}^2\paren{\Phiperp \hat\Phi^\top} \\
    &=: 1 - \dist\paren{\hat\Phi, \Phi_\star}.
\end{align*}
Now addressing the cross term, we have:
\begin{align*}
    \lambda_{\max}\paren{\Delta^\top F_\star^\top F_\star \Phi_\star \hat\Phi^\top + \hat\Phi \Phi_\star^\top F_\star^\top F_\star \Delta} &\leq 2\sigma_{\max}\paren{\Delta^\top F_\star^\top F_\star \Phi_\star \hat\Phi^\top} \\
    &\leq 2 \norm{\Delta} \norm{F_\star^\top F_\star} \norm{\Phi_\star \hat\Phi^\top} \\
    &\leq 2 \norm{\Phi_\star \paren{I - \hat\Phi^\top \hat\Phi}} \norm{\paren{\sum_{i=1}^N z_i z_i^\top } \hat\Phi^\top \paren{\sum_{i=1}^N \hat\Phi z_i z_i^\top \hat\Phi^\top }^{-1}} \norm{F_\star^\top F_\star} \\
    &\leq 2\; \dist\paren{\hat\Phi, \Phi_\star} \norm{F_\star^\top F_\star} \norm{\paren{\sum_{i=1}^N z_i z_i^\top } \hat\Phi^\top \paren{\sum_{i=1}^N \hat\Phi z_i z_i^\top \hat\Phi^\top }^{-1}}.
\end{align*}
To bound the term involving the empirical covariance, we can do something crude to yield
\begin{align*}
    \norm{\paren{\sum_{i=1}^N z_i z_i^\top } \hat\Phi^\top \paren{\sum_{i=1}^N \hat\Phi z_i z_i^\top \hat\Phi^\top }^{-1}} &\leq \frac{\norm{\frac{1}{N} \sum_{i} z_iz_i^\top } \norm{\hat\Phi}}{\lambda_{\min}\paren{\frac{1}{N} \sum_i \hat\Phi z_i z_i^\top \hat\Phi^\top}} \\
    &\leq \frac{\norm{\frac{1}{N} \sum_{i} z_iz_i^\top } }{\lambda_{\min}\paren{\frac{1}{N} \sum_i  z_i z_i^\top}} \\
    &\leq c \kappa\paren{\Sigma_z} \quad \text{with high probability},
\end{align*}
The last line comes from conditioning on the high-probability lower and upper isometry events $\underline c \lambda_{\min}(\Sigma_z) I \prec \frac{1}{N}\sum_i z_i z_i^\top \prec \overline c \lambda_{\max}(\Sigma_z) I$, and $c = \overline c / \underline c$ is some small numerical constant (e.g.\ $2$ or $1.1/0.9$ \citep{zhang2022multi}) that we control.  Therefore, plugging in our bounds on the dominant and cross terms back in, we have
\begin{align*}
    \norm{I - \eta F_+^\top F_+} &= 1 - 
\eta \lambda_{\min}\paren{F_+^\top F_+} \\
&\geq 1 - \eta \brac{\lambda_{\min}\paren{F_\star^\top F_\star} \paren{1 - \dist\paren{\hat\Phi, \Phi_\star}} - 2c\; \dist\paren{\hat\Phi, \Phi_\star} \norm{F_\star^\top F_\star} \kappa\paren{\Sigma_z} - \calO\paren{\frac{1}{\sqrt{N}}}}.
\end{align*}
This illustrates the intuition that once $\hat\Phi$ is close to the optimal $\Phi_\star$, and sufficient data $N$ is collected, then the nuisance terms will be much smaller than the primary contraction term. However, we must ensure that the initial representation $\hat\Phi_0$ is sufficiently close to $\Phi_\star$ to initialize the induction argument. \cite{tripuraneni2021provable} describes a method-of-moments estimator in the linear regression case, which \cite{collins2021exploiting} uses. \red{To do: adapt an initialization scheme to the matrix regression / operator recovery setting.}


\subsubsection{Bounding the Gram-Schmidt factor $\sigma_{\min}(R)$}

As discussed earlier, to bounding the Gram-Schmidt factor reduces to expanding $R R^\top = R\hat\Phi_+ \paren{R \hat\Phi_+}^\top$:
\begin{align*}
    R R^\top &= \paren{\hat\Phi - \eta F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star} - \eta \sum_{i=1}^N F_+^\top w_i z_i^\top \paren{\sum_{i=1}^N z_i z_i^\top}^{-1}} \\
    &\quad\cdot \paren{\hat\Phi - \eta F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star} - \eta \sum_{i=1}^N F_+^\top w_i z_i^\top \paren{\sum_{i=1}^N z_i z_i^\top}^{-1}}^\top \\
    &= I - \eta \hat\Phi\paren{F_+ \hat\Phi - F_\star \Phi_\star}^\top F_+ - \eta F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}\hat\Phi^\top + \eta^2  F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star} \paren{F_+ \hat\Phi - F_\star \Phi_\star}^\top F_+ + \calO\paren{\frac{1}{\sqrt{N}}}.
\end{align*}
Similar to our analysis in the previous section, we observe the term quadratic in the step size $\eta$ is psd and can only serve to help increase $\sigma_{\min}(R)$, and thus we toss it away; it remains to bound
\begin{align*}
    \lambda_{\max}\paren{\hat\Phi\paren{F_+ \hat\Phi - F_\star \Phi_\star}^\top F_+ + F_+^\top \paren{F_+ \hat\Phi - F_\star \Phi_\star}\hat\Phi^\top} = \lambda_{\max}\paren{2F_+^\top F_+ - \hat\Phi\Phi_\star^\top F_\star^\top F_+ - F_+^\top F_\star \hat\Phi \Phi_\star^\top }
\end{align*}


\subsubsection{Self-normalized martingale bounds and covering over $F_+$}

==> tex/practical_concerns.tex <==
\section{Practical Considerations}

Some desiderata to think about:
\begin{itemize}
    \item Extend algorithm to arbitrary composition of non-linear functions $\pi^{(h)}(x) = F^{(h)} \Phi x \rightarrow \pi^{(h)}(x) = f^{(h)}\circ \Phi(x)$. The overall algorithm should look similar to \Cref{alg: multi-task LIP}--this is analogous to the general schema of \texttt{FedRep}. Proving bounds will be out of the question.
    
    \item Centralized update occurring asynchronously. This can be seen as a version of \texttt{FedRep}'s analysis, where a sparse number of agents provide the directions for the representation update per iteration.
    
    \item Getting rid of the standard assumption that each system is initialized with a stabilizing controller; some recent work \red{cite some stuff} addresses this. We can afford to be dimension-suboptimal here, since its effect on regret asymptotically goes away.
    
    
\end{itemize}
